Contingency Planning Using Bi-level Markov Decision Processes for Space Missions

This work focuses on autonomous contingency planning for scientific missions by enabling rapid policy computation from any off-nominal point in the state space in the event of a delay or deviation from the nominal mission plan. Successful contingency planning involves managing risks and rewards, often probabilistically associated with actions, in stochastic scenarios. Markov Decision Processes (MDPs) are used to mathematically model decision-making in such scenarios. However, in the specific case of planetary rover traverse planning, the vast action space and long planning time horizon pose computational challenges. A bi-level MDP framework is proposed to improve computational tractability, while also aligning with existing mission planning practices and enhancing explainability and trustworthiness of AI-driven solutions. We discuss the conversion of a mission planning MDP into a bi-level MDP, and test the framework on RoverGridWorld, a modified GridWorld environment for rover mission planning. We demonstrate the computational tractability and near-optimal policies achievable with the bi-level MDP approach, highlighting the trade-offs between compute time and policy optimality as the problem's complexity grows. This work facilitates more efficient and flexible contingency planning in the context of scientific missions.

==> notes.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Extended abstract}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this paper we present a contingency planning procedure based on sparse Markov Decision Processes (MDPs). The framework we propose is general-purpose and designed to be used for any scientific mission. We further describe the specific application of this framework in generating contingency plans for NASA’s Volatiles Investigating Polar Exploration Rover (VIPER) during its planned mission to the lunar South Pole. Any scientific mission involves balancing multiple considerations such as time or cost constraints, as well as risks and scientific rewards associated, often probabilistically, with possible activities. A commonly used framework to model decision making in such scenarios is a Markov Decision Process (MDP). An MDP is characterized by a set of states, a set of actions, a probabilistic transition function from the current state to the next state, and a reward function resulting from taking each potential action at the current state. In scenarios such as traverse planning for VIPER, the action space and the planning horizon can be extremely large. For example, at each point within the traverse, the rover may move in multiple directions, with varying speeds depending on angle relative to sun and current science operations, as well as with multiple different goal targets for the next science station. For the most fine-grained planning, this would require actions to be taken every hour, while accumulating rewards over the total mission lifetime of over four months, i.e., a horizon of over 100,000 timesteps. It is therefore computationally intensive to generate the nominal planning policy and becomes even more challenging when generating multiple contingency plans in the event of specific failures. This intractability of the full fine-grained MDP planning motivates our work in using sparse and secondary MDPs for contingency planning. As our first contribution, we present a framework for handling mission planning with large action spaces and planning horizons. We propose a sparsification of the MDP by identifying a limited number of decision points and provide examples of such decision points specific to space missions. Additional complexity and greater optimality can be achieved by increasing the number of decision points or, as in our work, adding secondary MDPs in a bi-level framework. We compare our bi-level sparse MDP approach to the original fine-grained MDP in a large planning horizon and show that our approach is more computationally tractable while achieving near-optimal policies. In addition to comparing computational tractability and optimality, we also present, as our second contribution, a framework for comparing robustness against the original MDP. Our framework quantifies robustness specifically for space missions, where robustness is not only the absence of failure scenarios but also the reliable and risk-sensitive accumulation of scientific value. As our third and final contribution, we describe the application of this framework to generating contingency plans for VIPER and demonstrate the advantages of our framework in terms of computational tractability, near-optimality, and robustness.



This paper aims to introduce bi-level MDPs specifically for scientific mission planning, by describing how key decision points can be chosen to create a bi-level framework, and demonstrating the resulting improvement in tractability, which unlocks the ability to generate contingency plans from any arbitrary state.


The contributions of this paper are as follows: We introduce a modified GridWorld environment that captures the time-sensitive constraints in rover mission planning, which we call RoverGridWorld. We present a framework for handling mission planning with large action spaces and planning horizons. We show how a mission planning MDP can be converted into a bi-level MDP by identifying a limited number of decision points (or branching-off points). We compare our bi-level MDP approach to the original flat MDP, and show that our approach is more computationally tractable while achieving near-optimal policies. As the complexity of the problem increases, i.e., action spaces and state spaces get larger and time horizons get longer, we examine the trade-offs between computational complexity and optimality of the policy.


Motivation: 
\begin{itemize}
    \item space mission planning increasingly autonomous
    \item stochasticity is inherent
    \item risk/reward management is crucial
    \item problem can be formulated as MDP
    \item action space is very large, time horizon is very large compared to discretization of planning steps
    \item naturally lends itself to bi-level formulations (high-level strategic, low-level tactical)
    \item bi-level structure allows for introduction for human preferences, increasing acceptance and trustworthiness of AI solutions
\end{itemize}

Related work: \\
(1) other approaches to doing mission planning (and particularly traverse planning for rovers)
why is MDP best suited? why is bi-level MDP best suited?
(2) space mission planning is bi-level (cite VIPER planning paper?)
(3) other applications of bi-level MDP, e.g., cite paper for balancing EV charging load

Contributions:
(1) introduce bi-level framework, show near-optimality to fine-grained while reducing computation time
(2) show robustness?
(3) show applicability to VIPER?
Alternatively
(2) show adaptability to changing mission parameters/ model
    (2a) add in smg as a stochastic element
    (2b) modify science value "on-the-fly"
(3) robustness by adding a buffer required for the rover? effectively shifting the shadows? so the strategic plan remains the same, only temporal has to be recomputed.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Problem formulation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
inspiration = mission planning for a rover

our problem = modified grid world\\
key differences
\begin{itemize}
    \item transition always moves to intended direction. 
    \item time is a crucial component of state:\\
    \begin{itemize}
        \item many parts of the mission rely on being at the right place at the right time (e.g., science can only be done when not in comm shadow, reward function is time-dependent)
        \item many parts of the msision are time-sensitive (e.g., must make it to a safe haven before lunar night)
        \item many aspects of the environment change with time (e.g., sun direction changes, and speed depends on sun direction, so transition function is time-dependent)
        \item both transition and reward functions are time-dependent 
    \end{itemize}
    \item planning horizon is very large compared to time discretization, making state space also very large
\end{itemize}

Show the time-varying rewards in RoverGridWorld



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Approach}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Convert a fine-grained MDP to a bi-level MDP for mission planning (how to guide)

Formalize the math (algorithm blocks)

Show diagrams of strategic (HL MDP) vs tactical (LL MDP) planning

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Results}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Experiment 1: fine-grained vs bi-level 
optimality vs computation time

Experiment 2: testing adaptability by adding in smg stochasticity

Experiment 3: testing adaptability by adding in different obstacles/science rewards

Experiment 4: testing robustness by adding in different time buffers



\section{Contingency plans}
- in ideal world, just build one large tree
    - break up into nominal plan
    - and branches from off-nominal states
- for computation, we decide on branching-off states
    - how to derive the branching-off states: derived from the nominal plan
- state can get more complicated (energy included?)
    - the computation difference gets wider
- action complications
    - measurements take different times
    - smg stochasticity


\section{Discussion}
Some outcomes: 
longer paths to target locations
% https://ieeexplore.ieee.org/abstract/document/1545548
% "Furthermore, in some (but not all) cases the system can converge to somewhat longer paths to target locations than standard flat value iteration. This situation can arise because low-level value functions which are optimal with respect to reaching the next high-level state from the current high-level state are not always optimal with respect to reaching the final target state (see figure 2 for an illustration). It is also possible that high-level reward functions are not completely accurate because they average over low-level rewards. "

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Future directions}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this paper, we focused on the bi-level framework and what that unlocks. In the future, we would investigate a solver that can make use of this bi-level framework and do better than two separate value iterations. E.g. bi-level proximal policy optimization from \cite{long2019bi}.


Make time component of state continuous\\
% https://proceedings.neurips.cc/paper/2000/file/09b15d48a1514d8209b192a8b8f34e48-Paper.pdf\\
Time-Dependent MDP model 
where states have a discrete component (location) and real-valued time component


Consider adding a third intermediate level to the MDP that monitors for "safe exploration" in MDPs (Pieter Abbeel paper), i.e. removes unsafe actions from the low-level planner, to preserve ergodicity, and prevent catastrophic failure.
% https://arxiv.org/pdf/1205.4810.pdf
% Our framework quantifies robustness specifically for space missions, where robustness is not only the absence of failure scenarios but also the reliable and risk-sensitive accumulation of scientific value.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Notes/Expansions}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
https://ieeexplore.ieee.org/abstract/document/8920632
Bi-level MDP used to balance EV charging load with availability of wind power
	
	
bi-level mission planning is already a thing
- high-level targets identified in strategic planning
- tactical planning to get to each targets
this work
- formalizes, automates, and optimizes the process 
- reasons over stochasticity


